Embed to rigorously and accurately homogenise quasi-periodic multi-scale heterogeneous PDEs, with computer algebra

For microscale heterogeneous PDEs, this article further develops novel theory and methodology for their macroscale mathematical/asymptotic homogenization. This article specifically encompasses the case of quasi-periodic heterogeneity with finite scale separation: no scale separation limit is required. Dynamical systems theory frames the homogenization as a slow manifold of the ensemble of all phase-shifts of the heterogeneity. Depending upon any perceived scale separation within the quasi-periodic heterogeneity, the homogenization may be done in either one step, or two sequential steps: the results are equivalent. The theory not only assures us of the existence and emergence of the homogenization, it also provides a practical systematic method to construct the homogenization to any specified order. For a class of heterogeneities, we show that the macroscale homogenization is potentially valid down to lengths which are just twice that of the microscale heterogeneity! This methodology provides a new rigorous and flexible approach to homogenization that potentially also provides correct initial and boundary conditions, treatment of forcing and control, and analysis of uncertainty.

==> Figs/homoRadius.tex <==
% This file was created by matlab2tikz.
%
\tikzsetnextfilename{Figs/homoRadius}
\definecolor{mycolor1}{rgb}{0.13359,0.48867,0.73828}%
\definecolor{mycolor2}{rgb}{0.46758,0.53789,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
xmin=0,
xmax=0.25,
xlabel style={font=\color{white!15!black}},
xlabel={$1/n$},
ymin=2.8,
ymax=3.8,
ylabel style={font=\color{white!15!black}},
ylabel={$1/k_*^2$},
axis background/.style={fill=white},
width=100mm,height=40mm
]
\addplot [color=mycolor1, dotted, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
0.25	3.50139858386572\\
0.2	3.26518508995875\\
0.166666666666667	3.16899588685437\\
0.142857142857143	3.11855157366568\\
0.125	3.11116556288059\\
0.111111111111111	3.15343459085316\\
0.1	3.23515130526846\\
0.0909090909090909	3.32192259938042\\
0.0833333333333333	3.37862463490489\\
0.0769230769230769	3.39776559499579\\
0.0714285714285714	3.39722033691974\\
0.0666666666666667	3.40004684742514\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
0.25	2.8154840202015\\
0.2	2.97602265543671\\
0.166666666666667	3.08304841226018\\
0.142857142857143	3.15949538141981\\
0.125	3.21683060828952\\
0.111111111111111	3.26142467363264\\
0.1	3.29709992590713\\
0.0909090909090909	3.32628876867717\\
0.0833333333333333	3.35061280431886\\
0.0769230769230769	3.37119468063107\\
0.0714285714285714	3.38883628889868\\
0.0666666666666667	3.4041256827306\\
0	3.61817719637755\\
};
\end{axis}

\begin{axis}[%
xmin=0,
xmax=0.08,
xlabel style={font=\color{white!15!black}},
xlabel={$1/n^2$},
ymin=0.88,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$\cos2\theta_*$},
axis background/.style={fill=white},
width=100mm,height=40mm
]
\addplot [color=mycolor1, dotted, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
0.0625	0.978229282637076\\
0.04	0.959866923491973\\
0.0277777777777778	0.948073401277267\\
0.0204081632653061	0.935152377552595\\
0.015625	0.920120570704884\\
0.0123456790123457	0.905296380937195\\
0.01	0.895237565265754\\
0.00826446280991736	0.892583676936205\\
0.00694444444444444	0.894856958394094\\
0.00591715976331361	0.897318577105806\\
0.00510204081632653	0.897112987627055\\
0.00444444444444444	0.894200513122634\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
0.0625	0.997260495208701\\
0.04	0.956956751197994\\
0.0277777777777778	0.935063359389709\\
0.0204081632653061	0.921862334644453\\
0.015625	0.913294361853062\\
0.0123456790123457	0.907420187914601\\
0.01	0.903218425850385\\
0.00826446280991736	0.900109597111267\\
0.00694444444444444	0.897745077898313\\
0.00591715976331361	0.895904925951006\\
0.00510204081632653	0.894444821712\\
0.00444444444444444	0.893266884119346\\
0	0.885305650734515\\
};
\end{axis}
\end{tikzpicture}%
